Operator as a Service: Stateful Serverless Complex Event Processing

Complex Event Processing (CEP) is a powerful paradigm for scalable data management that is employed in many real-world scenarios such as detecting credit card fraud in banks. The so-called complex events are expressed using a specification language that is typically implemented and executed on a specific runtime system. While the tight coupling of these two components has been regarded as the key for supporting CEP at high performance, such dependencies pose several inherent challenges as follows. (1) Application development atop a CEP system requires extensive knowledge of how the runtime system operates, which is typically highly complex in nature. (2) The specification language dependence requires the need of domain experts and further restricts and steepens the learning curve for application developers. In this paper, we propose CEPLESS, a scalable data management system that decouples the specification from the runtime system by building on the principles of serverless computing. CEPLESS provides operator as a service and offers flexibility by enabling the development of CEP application in any specification language while abstracting away the complexity of the CEP runtime system. As part of CEPLESS, we designed and evaluated novel mechanisms for in-memory processing and batching that enables the stateful processing of CEP operators even under high rates of ingested events. Our evaluation demonstrates that CEPLESS can be easily integrated into existing CEP systems like Apache Flink while attaining similar throughput under a high scale of events (up to 100K events per second) and dynamic operator update in up to 238 ms.

==> Makefile <==
<<<<<<< HEAD
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'
=======
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'
>>>>>>> 9852529f80ddfdd55571083e9ab3a66b2ff8c4e3


==> sections/abstract_old.tex <==
% !TEX root = ./TCEP_main.tex


\begin{abstract}
Complex Event Processing (CEP) systems are widely employed in real-world scenarios %systems are widely used for real-world use cases 
such as fraud detection at financial institutions, 
%SEB bank, 
%(by Apama CEP processed at Software AG)
processing requests at e-commerce platforms
%(by Apache Flink 
%at Alibaba group 
and to manage tweets at Twitter. 
An \emph{operator} is an important foundation of a CEP system, which dictates computational units such as \emph{filter}, \emph{window}, etc., responsible for processing the incoming events. 
%among others
%It is 
%extremely important logical computational unit of a CEP system is an \emph{operator}, \eg \emph{filter}, \emph{window}, etc.,  which is responsible for processing incoming events. 
%Operators can be 
%A few examples of widely used operators are \emph{filter}, \emph{window}, \emph{join}, etc. 
%In CEP systems, the operators
The operators are often bound to their runtime environment and the respective programming language.
%\eg being offered by CEP systems like Apache Flink. 
This is extremely problematic for forenamed applications like fraud detection where it is highly essential to update an operator at runtime. %based on the application requirements. 
For instance, an operator meant for a specific user might not be as effective to detect fraud for another user due to different underlying conditions.
%an operator for fraud detection for a single user might not be able to detect fraud for multiple users because of different fraud conditions. 
Such functions need runtime updates of an operator in a CEP system. 
Furthermore, the reduced generality due to language dependence impedes the development of new user-defined operators. 
%Furthermore, language restrictions limit the universality with respect 
%of such operators.
%hamper advancement in development of operators for CEP systems.  

%(by Apache Storm). ACEP systems 
%https://www.progress.com/blogs/fighting-payment-fraud-with-complex-event-processing
%https://databricks.com/glossary/complex-event-processing
%https://www.gruenderszene.de/technologie/data-artisans-exit-alibaba
In this work, we address these problems by providing a serverless CEP architecture, \system, which offers 
%developers 
the flexibility to develop operators in any language and integrate them at runtime. 
%We embed operators in the function as a service model of serverless architecture. 
%In \system, we provide (i) a \emph{programming interface} to develop user-defined operators independent of the execution environment, (ii)  \emph{user-defined operator interface} for extending existing CEP systems and (iii) \emph{in-memory queue management} to maintain maximum throughput, highly essential for CEP systems. 
We show \system can be easily used in existing CEP systems like Apache Flink and matches the throughput and latency under high event rates of up to 100,000 events. 
We also simplify developing user-defined operators while benefiting from advanced features of CEP systems like Flink.
%This is very beneficial for applications like fraud detection where operators must be integrated at runtime to avoid service disruption. We show using our evaluation that our system  minimal overhead in latency, we can offer highly flexible server agnostic CEP operators.


% SH
%With operators being bound to the respective execution environments, CEP systems fail to fulfill the flexibility of complex applications which require different systems to interact together. Much like the microservice architecture, a streaming system could benefit from business logic written in different languages and architectures. For example, a current machine learning application which detects fraudulent customers is developed using a popular library only available in specific programming languages. However, if the streaming application does not provide the respective language bindings, this application needs to be adapted to the respective streaming engine. 



\end{abstract}

==> sections/background.tex <==
\section{Background}
In this section, we give a brief overview on the serverless paradigm.

%CEP is a paradigm which applies defined semantics to a flow of data items. These data items are notifications of events that happened in the external world and are observed by sources. \cite{Cugola2012} An event therefore can be seen as a physical or logical state change that occurred but is not limited to this \cite{snoop}. A CEP engine defines \textit{Producers} which pose as origin of data that is ingested into the system and \textit{Consumers} interested in meaningful events that are recognized by this system. CEP provides the ability to detect patterns in streams of events formulated by \textit{Queries}. In order to know if an item fulfills the patterns conditions, queries specify \textit{Operators}, which transform the event streams. A \textit{CEP engine} is used for parsing a query and supplying the operators for each part of operation. CEP engines build an acyclic directed graph based on the query whose root is the consumer. When the query is parsed and the operator graph has been built, the engine starts routing the incoming events from the producers through the graph to the consumer. \textit{Events} are identified as n-tuples \textit{(timestamp, value1, value2, ..., valueN)} containing information that the user specified by the issued query. These tuples are initially created and sent by the data producers in a system and often include raw data values as well as timestamps of the occurrence of the event.

Serverless or Function-as-a-Service (FaaS) is a compute paradigm that has evolved from compute providers such as Amazon Web Services (AWS). Serverless provides an abstraction for users to use services of a compute provider without direct knowledge of the underlying compute resource. This provides the serverless providers the ability to schedule serverless applications on any hardware suitable for the application and abstract away configuration complexity of the resources for users.

Using FaaS, users define functions executed by a provider which returns the result of the execution. A function is defined equivalent to functions in an executable application, however, the user needs to only submit the  code containing the function instead of a complete application. After submission, the provider is responsible for packaging and deploying the application, as well as receiving the results of the execution. 



==> sections/introduction_old.tex <==
% !TEX root = ./TCEP_main.tex

\section{Introduction} \label{sec:Introduction}
\mli{major: improve the motivation, remove the code example (was not very helpful, makes an impression of being rather easy) integrate the fraud detection example here. Clarify multiple aspects here: (i) the system is indeed able to provide benefits like any other serverless system -- automatic scaling and pay per use (per CEP function) with some extensions however the focus is on "function as a service" aspect in this paper. Justify better "the serverless" term. (ii) runtime update motivation needs to coupled with programming language independence more tightly, since there are existing tools for Java for example JRebel which allows runtime updates but are programming language dependent (in this case Java). Last review highlights some CEP engines that allows adding / modifying CEP rules on the fly, however, again they are runtime dependent and can execute only on this particular CEP system. Another option would be to change the motivation towards financial use case and remove Figure 1. (iii) clarify that we are more than a platform and in this context "server" means a "CEP runtime" which using our architecture reduces dependence on (of a UDO) (Fig 2b). (iv) It is definitely more than an implementation issue (need runtime updates) and the conceptual problems : the current CEP systems need to be understood before working on them (very hard to develop UDF operators) and rework on operators for different runtimes Flink vs Storm, it is difficult to compare them and lastly runtime updates and flexibility are much needed for current applications.}
\begin{comment}
\begin{enumerate}
    \item CEP introduction
    \item what is missing in current CEP system -- extreme complex design, one on one comparison in LOC of \system vs Flink. Highly dependent on the underlying server/system, system specific and language dependent.
    \item \system provides ... 
    \item \system platform for implementing user-defined operators which are system and programming language independent
    \item two case studies on open source CEP systems
    \item performance evaluation of \system in terms of latency, throughput and cpu load in different event rates
\end{enumerate}
\end{comment}

Complex Event Processing (CEP) is a powerful paradigm that can detect patterns in the data streams to derive higher level events. CEP systems can typically deal with high volume of events while delivering complex event detection in less than a few milliseconds. They are widely employed in real-world scenarios %systems are widely used for real-world use cases 
such as fraud detection at financial institutions. For instance, Apama CEP system  is currently used at SEB bank in Estonia to detect payment fraud\footnote{\url{https://www.progress.com/blogs/fighting-payment-fraud-with-complex-event-processing}}. Other prominent scenarios of CEP include processing requests for e-commerce platform Alibaba group 
%SEB bank, 
%(by Apama CEP processed at Software AG)
%processing requests at e-commerce platforms
%(by Apache Flink 
%at Alibaba group 
and managing tweets for Twitter using Apache Flink~\cite{flinkCarbone} and Storm~\cite{apacheHeron} respectively.
%\footnote{both Apache Flink and Storm are prominent open source CEP systems. \url{https://databricks.com/glossary/complex-event-processing}}.
An \emph{operator} is an important foundation of a CEP system that processes the incoming events in order to derive the higher level events. Some examples for these computational units are \emph{filter}, \emph{window}, among others. For instance, a filter \texttt{\{location = "Quebec"\}} checks the location of a user if the card terminal is same as user location in order to detect a fraud. 

Typically, the operators are tightly integrated (i) into a CEP system specialized for different runtime environments and (ii) to the respective domain-specific or main stream programming language of the CEP system. This is because conventional CEP systems provides a standard set of operators ranging from relational algebraic to logical operators~\cite{Cugola2012}. Current CEP systems like Flink provide a possibility to develop \emph{new} operators in the form of user-defined functions (UDFs). This feature provides a means to extend standard operators, however, UDFs need to be registered at compile time. 

%This restricts the possibility of runtime updates 
%among others
%It is 
%extremely important logical computational unit of a CEP system is an \emph{operator}, \eg \emph{filter}, \emph{window}, etc.,  which is responsible for processing incoming events. 
%Operators can be 
%A few examples of widely used operators are \emph{filter}, \emph{window}, \emph{join}, etc. 
%In CEP systems, the operators
%The operators are often bound to their runtime environment and the respective programming language.
%\eg being offered by CEP systems like Apache Flink. 
This is extremely problematic for aforementioned applications like fraud detection where it is extremely essential to update an operator at runtime. %based on the application requirements. 
For instance, an operator meant for a specific user might not be as effective to detect fraud for another user due to different underlying conditions. 
Simply because the pattern of transactions for a specific user might be completely different than of another user. Hence the two users may need a completely different pattern detection operator.
%an operator for fraud detection for a single user might not be able to detect fraud for multiple users because of different fraud conditions. 
Such functionality need runtime updates of an operator (e.g., for pattern detection) in a CEP system. Consider the example in \Cref{fig:case-study-intro}, on the left hand side (a) we present how a query in classical CEP systems like Flink is defined, wrapped into a jar and executed. 
A major drawback of this approach is that the query \codebox{highlighted} cannot be updated at runtime. 
However, often in such operators parameter updates are required, e.g., the threshold \texttt{0.78} could need an update. 
Rebuilding the CEP query is an option, but applications like fraud detection needs accurate and real-time detection of events and hence cannot afford to lose any data stream and time.  
Furthermore, the reduced generality due to language dependence impedes the development of new user-defined operators. 

\begin{figure*}
\centering
\includegraphics[width=0.8\linewidth]{figures/pdfs/case-study-intro.pdf}
\caption{An example of a simple financial fraud detection application (a) in classical CEP systems and (b) in \system system.}
\label{fig:case-study-intro} 
\end{figure*}

Hence, in this work we propose a serverless CEP architecture, \system, as described in \Cref{fig:case-study-intro} on the right hand side (b). 
The business logic of the operator as \codebox{highlighted} is segregated as a serverless CEP operator which (i) can be exchanged at runtime and (ii) is language independent. 
In this way, the CEP systems can benefit from  features of \emph{serverless computing}. 
However, a crucial research challenge we address in this work is to maintain (i) stateful processing of events and (ii) meet the latency and throughput requirements of forenamed applications while providing flexibility in the runtime. 
We enable this by providing \emph{in-memory queue management}, which ensures (i) stateful processing by maintaining the state in the queue and (ii) attain high throughput and low latency in processing by proposing \emph{pipelining} and \emph{batching} mechanisms.
In particular, we make the following contributions: 

\begin{enumerate}
    \item A \emph{programming interface} to develop user-defined operators and submit them to a registry using docker tools. 
    \item A \emph{user-defined operator interface} to facilitate communication of the existing CEP systems with \system platform. 
    \item \emph{In-memory queue management} for stateful processing and fast delivery of events as per the requirements of the applications.
    \item Implementation and evaluation of \system on two state-of-the art CEP systems \emph{Apache Flink}~\cite{flinkCarbone} and \emph{TCEP}~\cite{Luthra2018}, which enables runtime updates of user-defined operators through \system while matching the throughput and latency under high event rates of up to 100,000 events.
\end{enumerate}

We have structured the paper as follows. In \Cref{sec:casestudy}, we elaborate on the fraud detection case study and its challenges. In \Cref{sec:model}, we present the system model introducing the important system entities. In \Cref{sec:design}, we present the \system design. In \Cref{sec:evaluation} and \Cref{sec:conclusion} we present the evaluation and the conclusion, respectively.

%Furthermore, language restrictions limit the universality with respect 
%of such operators.
%hamper advancement in development of operators for CEP systems.  


%This is very beneficial for applications like fraud detection where operators must be integrated at runtime to avoid service disruption. We show using our evaluation that our system  minimal overhead in latency, we can offer highly flexible server agnostic CEP operators.


% SH
%With operators being bound to the respective execution environments, CEP systems fail to fulfill the flexibility of complex applications which require different systems to interact together. Much like the microservice architecture, a streaming system could benefit from business logic written in different languages and architectures. For example, a current machine learning application which detects fraudulent customers is developed using a popular library only available in specific programming languages. However, if the streaming application does not provide the respective language bindings, this application needs to be adapted to the respective streaming engine. 


%(by Apache Storm). ACEP systems 
%https://www.progress.com/blogs/fighting-payment-fraud-with-complex-event-processing
%https://databricks.com/glossary/complex-event-processing
%https://www.gruenderszene.de/technologie/data-artisans-exit-alibaba
%In this work, we address these problems by providing a serverless CEP architecture, \system, which offers 
%developers 
%the flexibility to develop operators in any language and integrate them at runtime. 
%We embed operators in the function as a service model of serverless architecture. 
